Knowledge Distillation for Real-Time Classification of Early Media in Voice Communications

This paper investigates the industrial setting of real-time classification of early media exchanged during the initialization phase of voice calls. We explore the application of state-of-the-art audio tagging models and highlight some limitations when applied to the classification of early media. While most existing approaches leverage convolutional neural networks, we propose a novel approach for low-resource requirements based on gradient-boosted trees. Our approach not only demonstrates a substantial improvement in runtime performance, but also exhibits a comparable accuracy. We show that leveraging knowledge distillation and class aggregation techniques to train a simpler and smaller model accelerates the classification of early media in voice calls. We provide a detailed analysis of the results on a proprietary and publicly available dataset, regarding accuracy and runtime performance. We additionally report a case study of the achieved performance improvements at a regional data center in India.

==> figs/map.tex <==
\begin{table}[H]
\center


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\resizebox{\linewidth}{!}{

    \begin{tabular}{ccccccc}
    \multicolumn{2}{l}{\multirow{2}{*}{}}                                                                                             & \multicolumn{4}{c}{Class}                                                                                                           \\ \cline{3-6} 
     \multicolumn{2}{l|}{} & \multicolumn{1}{l|}{Music} & \multicolumn{1}{l|}{Ringing} & \multicolumn{1}{l|}{Silence} & \multicolumn{1}{l|}{Announcement} & \multicolumn{1}{l}{mAP}  \\ \cline{2-7} 
    \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Model\end{tabular}}} & \multicolumn{1}{l|}{GBT}  & \multicolumn{1}{l|}{0.434}    & \multicolumn{1}{l|}{0.096}     & \multicolumn{1}{l|}{0.025}       & \multicolumn{1}{l|}{0.211}     & \multicolumn{1}{l|}{0.193}   \\ \cline{2-7} 
    \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{CNN14} & \multicolumn{1}{l|}{0.454}        & \multicolumn{1}{l|}{0.101}         & \multicolumn{1}{l|}{0.025}           & \multicolumn{1}{l|}{0.218}     &  \multicolumn{1}{l|}{0.200}  \\ \cline{2-7} 
    \end{tabular}
}
\caption{Average precision per class and mean average precision on a subset of audioset.}
\label{tab::map}
\end{table}

==> sections/problem_definition.tex <==

\section{Problem setting}
As previously mentioned, a common method when facilitating VoIP calls is the usage of SIP codes \cite{goode2002voice,rfc3261,johnston2015sip}. Figure \ref{fig::standard-sip-exchange} illustrates a typical exchange of SIP requests and responses exchanged between a caller's and callee's device prior to establishing a voice call. In practice these exchanges are facilitated through proxy SIP servers or SIP-based and public switched telephone network (PSTN) gateways.

% KEMAL: koment. Odlučio sam vratiti ovaj disclaimer gore, nadam se da je to okej. Jednostavno kako je prije stajalo djelovalo mi je da na slici nedostaju komponente ukoliko se ne naglasi.

%As shown in Fig. \ref{fig::standard-sip-exchange},  a typical exchange between SIP requests happens between a caller's and callee's devices usually through a SIP proxy server and either a SIP-based or public switched telephone network (PSTN) gateway. 
%These details were omitted from the diagram for simplicity. 
As shown on Figure 1, after receiving an initial \textit{invite} request to establish a call, the callee's side usually responds with \textit{100 trying} followed by \textit{180 ringing} code. In this work, we focus on the event that happens after these two responses have been sent. That is, if the callee accepts the call, the response will typically be \textit{200 OK}. After this response, the two devices begin exchanging media (call content) \cite{rfc3261,johnston2015sip}.

\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{figs/sip-exchange.pdf}
    \caption{Simplified diagram depicting exchanged SIP requests and responses during setup of a VoIP call.}
    \label{fig::standard-sip-exchange}
\end{figure}


However, in the case when the callee's side does not respond with a successful status (i.e, any response code starting with the number $2$), the SIP protocol defines several response codes that should be sent in a similar manner like HTTP. For example, these can be \textit{480 temporarily unavailable}, \textit{486 busy here}, \textit{502 bad gateway}, \textit{503 service unavailable} or \textit{608 rejected}, among others.
To be more specific, any response starting with numbers $3$, $4$, $5$ or $6$ indicates that something is preventing a successful call establishment. 
Handling such error codes successfully is important in the telecommunications domain as these impact the previously mentioned ASR \cite{ITUrecE425} metric.
Depending on the received SIP response in case it was not \textit{200 OK}, the caller's side can act upon them and attempt to establish the connection again. For example, reaching the callee can be attempted via another gateway.

%As already mentioned, a key metric defined by the International Telecommunication Union Standardization sector (ITU-T) is the ASR \cite{ITUrecE425}, which reflects the percentage of successful call connections compared to totall call attempts. Obviously, depending on which SIP responses were received other than \textit{200 OK}, the caller's side can act upon them and attempt to establish the connection again. For example, reaching the callee can be attempted via another gateway.

\vspace{2mm} \noindent 
%\subsection{Inconsistent SIP responses}
\textbf{Inconsistent SIP responses.} 
Within the scope of Infobip, one of the major cloud-communication platforms, we observed frequent cases where some telecommunication providers do not properly manage SIP responses. For example, regardless of the actual issue at hand a common case is that the same SIP code is always propagated in the response. However, we also noticed that some form of feedback is provided through early media. Such a setting provides an opportunity to analyze the content of early media and based on that content decide on what action to perform next e.g., perform a redial or try another gateway.
An example of such an early media audio is provided by Figure \ref{fig::sample-announcement}. The issue in this example is that the callee is out of the network coverage area and this information was encapsulated as a voice message. In this paper, we'll refer to such voice messages that contain useful information as \textit{early media announcements}.

%The issue which has motivated the authors of this paper is that some telecommunication providers do not properly manage SIP responses, e.g. regardless of the actual issue at hand they always propagate the same SIP response. We've observed that some of them do, however, provide some form of feedback through early media. Thus, we can analyze the content of early media and based on the content decide on which action to perform: redial, try another gateway, etc.



\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figs/waveform.pdf}
    \caption{{Example of an announcement sent as early media that contains information regarding the call. The transcript of this file is: "\textit{The number you are calling is out of network coverage area. Please try later."}. In this work we tackle the problem of mapping such an incoming voice message to the appropriate SIP code.}}
    \label{fig::sample-announcement}
\end{figure}


\vspace{2mm} \noindent 
\textbf{Matching Early Media Announcements.}
Extracting useful information from an early media announcement is a non-trivial task and beyond the scope of this paper. But we provide a few possible approaches to this problem. One is to apply automatic speech recognition and then extract the information from the transcript. This means mapping the transcripts to appropriate SIP codes. For regions with smaller VoIP traffic and fewer TSPs the number of different early media announcements in circulation and their variance is lower, thus another approach could be utilizing a simple keyword spotting algorithm \cite{sainath2015convolutional,navon2024open}.
Yet another strategy is to record samples of early media and assign them appropriate SIP codes (either manually or automatically) and add them to an audio retrieval database beforehand \cite{haitsma2002highly,wang2003industrial,baluja2008waveprint}. Once completed, this would enable us to query the audio retrieval database with any incoming early media in order to obtain the SIP code it is associated with. We've opted for the last approach and use an audio fingerprinting system similar to Shazam \cite{wang2003industrial} and Waveprint \cite{baluja2008waveprint} for efficiently storing and retrieving early media announcements.


\vspace{2mm} \noindent 
\textbf{Early Media Classification.}
There are two requirements for the previously mentioned retrieval of early media announcements. First of all, it must operate in real-time, scaling to a large number of parallel calls (e.g. $1,000$ simultaneous calls). The real-time requirement is necessary, as obtaining the information about an early media is not of any use if we try routing to another gateway after, for example, $30$ minutes as we desire to establish calls in a quickly manner.

The second requirement is that we must know whether the early media contains an announcement at all, as non-announcements cannot be mapped to an appropriate SIP code, so attempting to retrieve them from the audio database would not yield any benefits. Running the audio fingerprinting algorithm per every received early media also quickly becomes computationally expensive given the large volume of VoIP traffic and would require a lot of computational power to maintain its real-time operational mode. 
In our setting, we also observed that performing such an operation is redundant most of the time, as a significant portion of early media does not contain an announcement. This can be seen in Figure \ref{fig::early-media-labels-distribution}, where we show the class distribution of a $30$ day sample that contains 30 million early media voice messages.

Given the preceding discussion, we define the main task we tackle in this paper as: \textit{low-resource requirements classification of early media in real-time}. By applying the classification procedure on incoming early media beforehand and only running the fingerprinting algorithm for early media classified as \textit{announcements}, as we later show, we manage to increase the number of concurrent calls that we can handle by a factor of $3.11$. This also leads to an improvement in ASR \cite{ITUrecE425}, as we are able extract information from early media and try to redial unsuccessful call establishments.

%The previously mentioned retrieval of early media announcement is knowing the correct class of the voice message in real-time (e.g., is it an announcement or something else). For example, obtaining the information about an early media is not of any use if we try routing to another gateway after 30 minutes as we desire to establish calls in a quickly manner.

%In the following sections, we provide the details to our approach: classifying early media with the constraint of solving this problem in real-time while minimizing the computational power required by our solution.


\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figs/CLASS_bar_chart.pdf}
     \caption{Distribution of early media per four main classes we observed in Infobip across multiple regional datacenters over a span of $30$ days. Only about a quarter of the $30,000,000$ early media sample contain relevant announcements.}
    \label{fig::early-media-labels-distribution}
\end{figure}


==> todo.tex <==
1. Prepraviti reference (po uzoru na AMD rad)
2. Dodati grafik i section "Problem definition"
3. Testirati na public datasetu
4. Preći kroz dijelove opisa modela i feature extraction-a
5. factor improvementa
Na DC-u je 74\% early media non-announcement. Average runtime 77.81
ostatak se runa 5.6sec u average-u. Sada je average runtime .26*77.81 + 0.26*5.6, odnosno average runtime je 24.37ms, što je improvement sa faktorom od 3.19.

Neke bolje metrike umjesto samo confusion matrice na našem test setu.
